Real-time Visualization of Stream-based Monitoring Data

Stream-based runtime monitors are used in safety-critical applications such as Unmanned Aerial Systems (UAS) to compute comprehensive statistics and logical assessments of system health that provide the human operator with critical information in hand-over situations. In such applications, a visual display of the monitoring data can be much more helpful than the textual alerts provided by a more traditional user interface. This visualization requires extensive real-time data processing, which includes the synchronization of data from different streams, filtering and aggregation, and priorization and management of user attention. We present a visualization approach for the \rtlola monitoring framework. Our approach is based on the principle that the necessary data processing is the responsibility of the monitor itself, rather than the responsibility of some external visualization tool. We show how the various aspects of the data transformation can be described as RTLola stream equations and linked to the visualization component through a bidirectional synchronous interface. In our experience, this approach leads to highly informative visualizations as well as to understandable and easily maintainable monitoring code.

==> showcase.tex <==
\section{Showcase}\label{sec:showcase}


==> specification32.tex <==
\begin{lstlisting}
    import math
    input pixel_scale: (Float64, Float64)
    input charge: Float64
    input gps: (Float64, Float64)
    
    // filter out readings during initialization
    output filtered_gps
      filter gps != (0.0,0.0)
    := gps
    
    // create a smoothed GPS signal if we got at least one reading in this time frame
    output received_gps @ 1Hz
    := filtered_gps.aggregate(over: 2s, using: count) > 0
    output smoothed_gps @ 1Hz
      filter received_gps
    := filtered_gps.aggregate(over: 2s, using: average).defaults(to: start_position) 
    
    // simply use the global min/max per axis
    output x_limits: (Float64, Float64) 
      @ 1Hz
      filter received_gps
    := (min(smoothed_gps.0, x_limits.offset(by: -1).defaults(to: smoothed_gps).0),
        max(smoothed_gps.0, x_limits.offset(by: -1).defaults(to: (0.0,smoothed_gps.0)).1))
    output y_limits: (Float64, Float64) 
      @ 1Hz
      filter received_gps
    := (min(smoothed_gps.1, y_limits.offset(by: -1).defaults(to: (smoothed_gps.1,0.0)).0),
        max(smoothed_gps.1, y_limits.offset(by: -1).defaults(to: smoothed_gps).1))
    
    output pixel_scale_sampled @ 1Hz := pixel_scale.hold(or: 0.0)
    output gps_sampled @ 1Hz  := smoothed_gps.hold(or: start_position)
    output last_transferred_gps := if send_values then gps_sampled else last_transferred_gps.offset(by: -1).defaults(to: gps_sampled) 
    
    output x_normalized := (gps_sampled.0 - x_limits.hold(or: (0.0,1.0)).0) / (x_limits.hold(or: (0.0,1.0)).1 - x_limits.hold(or: (0.0,1.0)).0) 
    output y_normalized := (gps_sampled.1 - y_limits.hold(or: (0.0,1.0)).0) / (y_limits.hold(or: (0.0,1.0)).1 - y_limits.hold(or: (0.0,1.0)).0)
    output x_normalized_last := (last_transferred_gps.offset(by: -1).defaults(to: (gps_sampled.0 + tau,0.0)).0 - x_limits.hold(or: (0.0,1.0)).0) / (x_limits.hold(or: (0.0,1.0)).1 - x_limits.hold(or: (0.0,1.0)).1) 
    output y_normalized_last := (last_transferred_gps.offset(by: -1).defaults(to:(0.0, gps_sampled.1 + tau)).1 - y_limits.hold(or: (0.0,1.0)).0) / (y_limits.hold(or: (0.0,1.0)).1 - y_limits.hold(or: (0.0,1.0)).0) 
    
    output pixel_x := x_normalized * pixel_scale_sampled.0
    output pixel_y := y_normalized * pixel_scale_sampled.1
    output pixel_x_last := x_normalized_last * pixel_scale_sampled.0
    output pixel_y_last := y_normalized_last * pixel_scale_sampled.1
    
    constant start_position : (Float64, Float64) := (0.0, 0.0)
    constant tau: Float64 := 10.0
    output send_values @ 1Hz 
    := sqrt((pixel_x - pixel_x_last)**2.0 + (pixel_y - pixel_y_last)**2.0) > tau
        $\land$ received_gps
    
    // use tuple to ensure synchronized data
    output marker: (Float64, Float64, Float64)
        @ 1Hz
        filter send_values
    := (filtered_gps.hold(or: start_position).0, filtered_gps.hold(or: start_position).1,charge.hold(or: 100.0))
    \end{lstlisting}
